Task-Aware Network Coding Over Butterfly Network

Network coding allows distributed information sources such as sensors to efficiently compress and transmit data to distributed receivers across a bandwidth-limited network. Classical network coding is largely task-agnostic -- the coding schemes mainly aim to faithfully reconstruct data at the receivers, regardless of what ultimate task the received data is used for. In this paper, we analyze a new task-driven network coding problem, where distributed receivers pass transmitted data through machine learning (ML) tasks, which provides an opportunity to improve efficiency by transmitting salient task-relevant data representations. Specifically, we formulate a task-aware network coding problem over a butterfly network in real-coordinate space, where lossy analog compression through principal component analysis (PCA) can be applied. A lower bound for the total loss function for the formulated problem is given, and necessary and sufficient conditions for achieving this lower bound are also provided. We introduce ML algorithms to solve the problem in the general case, and our evaluation demonstrates the effectiveness of task-aware network coding.

==> figs_tex/architecture.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.65]{figs/butterfly.pdf}
\caption{Task-aware network coding over butterfly network.}
\label{fig:architecture}
\end{figure}

==> figs_tex/explanation.tex <==
\begin{figure*}[t]
\centering
% \includegraphics[scale=1]{figs/explanation.pdf}
\begin{align}
& W 
=
\begin{bmatrix}
v_{r_+^{(3,4)}-2Z+1}^\top\\
v_{r_+^{(3,4)}-2Z+2}^\top\\
\vdots\\
v_{2Z}^\top
\end{bmatrix}
\xrightarrow[n-b+1:a,\text{ Gauss-Jordan elimination}]{\text{Step I: }\text{put columns }a+1:n\text{ before }}\notag
\begin{array}{r}
{\scriptstyle n-b'}\{\\
{\scriptstyle n-a'}\{\\
{\scriptstyle r_-^{(3,4)} + a'+b'-2n}\{\\
\end{array}
\left[
\begin{array}{c|c|c}
\ast &\ast & \ast \\ \hline
0 & \ast & \ast\\ \hline
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{1:n-b}} & 
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{a+1:n}} &
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}\ast}_{n-b+1:a}}
\end{array}\right]
\xrightarrow
[a+1:n\text{ before }1:n-b,]
{\text{Step II: }\text{put columns }}
\\[1em]
& 
\xrightarrow
[\text{for the first }n-b'\text{ rows}]
{\text{Gauss-Jordan elimination}}
\notag
\begin{array}{r}
{\scriptstyle \min\{a'-a, n - b'\}}\{\\
{\scriptstyle \max\{n-b'-a'+a, 0\}}\{\\
{\scriptstyle n-a'}\{\\
{\scriptstyle r_-^{(3,4)} + a'+b'-2n}\{\\
\end{array}
\left[
\begin{array}{c|c|c}
\ast & \ast & \ast \\ \hline
0 & \ast & \ast\\ \hline
\ast & 0 & \ast\\ \hline
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{a+1:n}} & 
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{1:n-b}} & 
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}\ast}_{n-b+1:a}}
\end{array}\right]
\xrightarrow[\text{rearrange}]{\text{Step III}}
\left[
\begin{array}{c|c|c}
 \ast & \ast & \ast \\ \hline
 \ast & \ast & 0 \\ \hline
0 & \ast & \ast\\ \hline
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{1:n-b}} & 
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}\ast}_{n-b+1:a}} &
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{a+1:n}}
\end{array}\right]
\begin{array}{l}
\leftarrow {\scriptstyle G_1}\\
\leftarrow {\scriptstyle G_2}\\
\leftarrow {\scriptstyle G_3}\\
\leftarrow {\scriptstyle G_4}
\end{array}
\notag
\end{align}
\caption{Explanation for the proof of Theorem \ref{thm:sf3}. Here $0$ and $\ast$ represent submatrices that must and may not contain only zero elements, respectively. The notations at the bottom represent the column indices, and the notations on the left represent the number of rows.}
\label{fig:explanation}
\end{figure*}

==> figs_tex/mnist_evaluation.tex <==
\begin{figure*}[t]
\centering

% \input{figs_tikz/legend_approaches.tex}

% \subfigure{
% \input{figs_tikz/mnist_test_loss_bottleneck.tex}
% \label{fig:loss_bottleneck}
% }
% \subfigure{
% \input{figs_tikz/mnist_test_loss_comparison.tex}
% \label{fig:eval_comparison}
% }

\begin{minipage}[t]{0.6\linewidth}
\strut\vspace*{-\baselineskip}\newline
\subfigure{
\hspace{0.08\linewidth}
\input{figs_tikz/legend_approaches_two_row.tex}
}
\addtocounter{subfigure}{-1}
\subfigure[]{
\input{figs_tikz/mnist_test_loss_bottleneck.tex}
\label{fig:mnist_loss_bottleneck}
}
\subfigure[]{
\input{figs_tikz/mnist_test_loss_weight.tex}
\label{fig:mnist_loss_weight}
}
\end{minipage}\hfill
\begin{minipage}[t]{0.35\linewidth}
\strut\vspace*{-\baselineskip}\newline
\subfigure[]{
\input{figs_tikz/mnist_test_loss_comparison.tex}
\label{fig:mnist_loss_comparison}
}
\end{minipage}

\caption{Evaluation result with MNIST dataset. Left: overall task loss $\mathcal{L}_\text{total}$ under different edge capacity $Z$ (with $\gamma = 0.9$).  Middle: overall task loss $\mathcal{L}_\text{total}$ under different weight $\gamma$ (with $Z = 10$). Right: comparison of the utilities of $\phi^{(5,6)}, \phi^{(1,3)}$ and $\phi^{(2,4)}$ for different approaches (with $Z=10$ and $\gamma=0.9$).}
\label{fig:mnist_evaluation}
\end{figure*}

==> figs_tex/obs.tex <==
\begin{figure}[t]
\centering
% \includegraphics[scale=0.5]{figs/data_and_task.pdf}
$\underbrace{x_1, \cdots, x_{n-b}, \lefteqn{\overbrace{\phantom{x_{n-b+1} \cdots, x_a, x_{a+1}, \cdots, x_n}}^{x^{(2)}}} x_{n-b+1}, \cdots, x_a, }_{x^{(1)}} x_{a+1}, \cdots, x_n$\\
% $\underbrace{x_{s_1}, \cdots, x_{s_{n-d}}, \lefteqn{\overbrace{\phantom{x_{s_{n-d+1}} \cdots, x_{s_c}, x_{s_{c+1}}, \cdots, x_{s_n}}}^{\text{related to } K^{(4)}}} x_{s_{n-d+1}}, \cdots, x_{s_c}, }_{\text{related to } K^{(3)}} x_{s_{c+1}}, \cdots, x_{s_n}$
\caption{Observations.}
\label{fig:obs}
\end{figure}

==> figs_tex/old/architecture.tex <==
\begin{figure*}[t]
\centering
\includegraphics[scale=0.7]{figs/formulation.pdf}
\caption{Architecture.}
\label{fig:architecture}
\end{figure*}

==> figs_tex/old/architecture_2.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.65]{figs/butterfly.pdf}
\caption{Task-aware network coding over butterfly network.}
\label{fig:architecture}
\end{figure}

==> figs_tex/old/evaluation1.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{figs/theory_test_bottleneck.pdf}
\caption{Evaluation result 1.}
\label{fig:eval1}
\end{figure}

==> figs_tex/old/explanation.tex <==
\begin{figure*}[t]
\centering
% \includegraphics[scale=1]{figs/explanation.pdf}
\begin{align}
& W 
=
\begin{bmatrix}
v_{r_+^{(3,4)}-2Z+1}^\top\\
v_{r_+^{(3,4)}-2Z+2}^\top\\
\vdots\\
v_{2Z}^\top
\end{bmatrix}
\xrightarrow[\text{put columns }a+1:n\text{ before }n-b+1:a]{\text{Step I}}
\left[
\begin{array}{c|c|c}
& &\\
\ast &\ast & \ast\\
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}}_{1:n-b}} & 
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}}_{a+1:n}} &
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}}_{n-b+1:a}}
\end{array}\right]
\xrightarrow[\text{Gauss-Jordan elimination}]{\text{Step II}}\notag\\[1em]
&
\begin{array}{r}
{\scriptstyle n-b'}\{\\
{\scriptstyle n-a'-p}\{\\
{\scriptstyle r_-^{(3,4)} + a'+b'+p-2n}\{\\
\end{array}
\left[
\begin{array}{c|c|c|c}
\ast &\ast & 0 & \ast \\ \hline
0 & 0 & \ast & \ast\\ \hline
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{1:n-b}} & 
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{a+1:a+p}} &
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{a+p+1:n}} &
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}\ast}_{n-b+1:a}}
\end{array}\right]
\xrightarrow
[\text{then Gauss-Jordan elimination for the first }n-b\text{ rows}]
{\text{Step III: }\text{put columns }a+1:n\text{ before }1:n-b,}
\notag\\[3em] 
& 
\begin{array}{r}
{\scriptstyle \min\{p, n - b'\}}\{\\
{\scriptstyle \max\{n-b'-p, 0\}}\{\\
{\scriptstyle n-a'-p}\{\\
{\scriptstyle r_-^{(3,4)} + a'+b'+p-2n}\{\\
\end{array}
\left[
\begin{array}{c|c|c|c}
\ast & 0 & \ast & \ast \\ \hline
0 & 0 & \ast & \ast\\ \hline
0 & \ast & 0 & \ast\\ \hline
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{a+1:a+p}} &
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{a+p+1:n}} & 
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{1:n-b}} & 
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}\ast}_{n-b+1:a}}
\end{array}\right]
\xrightarrow[\text{rearrange}]{\text{Step IV}}
\left[
\begin{array}{c|c|c}
 \ast & \ast & \ast \\ \hline
 \ast & \ast & 0 \\ \hline
0 & \ast & \ast\\ \hline
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{1:n-b}} & 
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}\ast}_{n-b+1:a}} &
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{a+1:n}}
\end{array}\right]
% \begin{array}{l}
% \}{\scriptstyle p}\\
% \}{\scriptstyle n-b-p}\\
% \}{\scriptstyle n-a-p}\\
% \}{\scriptstyle r_-^{(3,4)} + a+b+p-2n}\\
% \end{array}
\notag\\[3em] 
&
\xrightarrow[\text{division}]{\text{Step V}}
\begin{array}{r}
{\scriptstyle \min\{p, n - b'\}}\{\\
{\scriptstyle \max\{n-b'-p, 0\}}\{\\
{\scriptstyle n-a'-p}\{\\
{\scriptstyle |n-a'-p - \max\{n-b'-p, 0\}|}\{\\
% {\scriptstyle Z-n+a'+p-\min\{p,n-b'\}}\{\\
{\scriptstyle r_-^{(3,4)} + a'+b'+p-2n - |n-a'-p - \max\{n-b'-p, 0\}|}\{
\end{array}
\left[
\begin{array}{c|c|c}
 \ast & \ast & \ast \\ \hline
 \ast & \ast & 0 \\ \hline
0 & \ast & \ast\\ \hline
0 & \ast & 0\\ \hline
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{1:n-b}} & 
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}\ast}_{n-b+1:a}} &
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{a+1:n}}
\end{array}\right]
\begin{array}{l}
\leftarrow {\scriptstyle \text{Group 1}}\\
\leftarrow {\scriptstyle \text{Group 2}}\\
\leftarrow {\scriptstyle \text{Group 3}}\\
\leftarrow {\scriptstyle \text{Group 2 if } a'\leq b' \text{; Group 3 o.w.}}\\
\leftarrow {\scriptstyle \text{Group 4}}
\end{array}
\notag
\end{align}
\caption{Explanation for the proof of Theorem \ref{thm:sf3}. Here $0$/$\ast$ means a sub matrix must/may not contain only zero elements, the notations at the bottom represent the column indices, and the notations on the left represent the number of rows.}
\label{fig:explanation}
\end{figure*}

==> figs_tex/old/explanation_2.tex <==
\begin{figure*}[t]
\centering
% \includegraphics[scale=1]{figs/explanation.pdf}
\begin{align}
& W 
=
\begin{bmatrix}
v_{r_+^{(3,4)}-2Z+1}^\top\\
v_{r_+^{(3,4)}-2Z+2}^\top\\
\vdots\\
v_{2Z}^\top
\end{bmatrix}
\xrightarrow[\text{put columns }a+1:n\text{ before }n-b+1:a]{\text{Step I}}
\left[
\begin{array}{c|c|c}
& &\\
\ast &\ast & \ast\\
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}}_{1:n-b}} & 
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}}_{a+1:n}} &
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}}_{n-b+1:a}}
\end{array}\right]
\xrightarrow[\text{Gauss-Jordan elimination}]{\text{Step II}}\notag\\[1em]
&
\begin{array}{r}
{\scriptstyle n-b'}\{\\
{\scriptstyle n-a'}\{\\
{\scriptstyle r_-^{(3,4)} + a'+b'-2n}\{\\
\end{array}
\left[
\begin{array}{c|c|c}
\ast &\ast & \ast \\ \hline
0 & \ast & \ast\\ \hline
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{1:n-b}} & 
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{a+1:n}} &
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}\ast}_{n-b+1:a}}
\end{array}\right]
\xrightarrow
[\text{then perform Gauss-Jordan elimination for the first }n-b'\text{ rows}]
{\text{Step III: }\text{put columns }a+1:n\text{ before }1:n-b,}
\notag\\[3em] 
& 
\begin{array}{r}
{\scriptstyle \min\{a'-a, n - b'\}}\{\\
{\scriptstyle \max\{n-b'-a'+a, 0\}}\{\\
{\scriptstyle n-a'}\{\\
{\scriptstyle r_-^{(3,4)} + a'+b'-2n}\{\\
\end{array}
\left[
\begin{array}{c|c|c}
\ast & \ast & \ast \\ \hline
0 & \ast & \ast\\ \hline
\ast & 0 & \ast\\ \hline
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{a+1:a+n}} & 
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{1:n-b}} & 
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}\ast}_{n-b+1:a}}
\end{array}\right]
\xrightarrow[\text{rearrange}]{\text{Step IV}}
\left[
\begin{array}{c|c|c}
 \ast & \ast & \ast \\ \hline
 \ast & \ast & 0 \\ \hline
0 & \ast & \ast\\ \hline
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{1:n-b}} & 
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}\ast}_{n-b+1:a}} &
\smash{\underbrace{\vphantom{\rule[-1em]{0pt}{0pt}}0}_{a+1:n}}
\end{array}\right]
\begin{array}{l}
\leftarrow {\scriptstyle G_1}\\
\leftarrow {\scriptstyle G_2}\\
\leftarrow {\scriptstyle G_3}\\
\leftarrow {\scriptstyle G_4}
\end{array}
\notag
\end{align}
\caption{Explanation for the proof of Theorem \ref{thm:sf3}. Here $0$ and $\ast$ represent submatrices that must and may not contain only zero elements, respectively. The notations at the bottom represent the column indices, and the notations on the left represent the number of rows.}
\label{fig:explanation}
\end{figure*}

==> figs_tex/old/network_coding.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.65]{figs/network_coding.pdf}
\caption{Network coding over butterfly network.}
\label{fig:network_coding}
\end{figure}

==> figs_tex/old_2/synthetic_evaluation.tex <==
\begin{figure}[t]
\centering

% \subfigure[]{
% \input{figs_tikz/synthetic_test_loss_r34+.tex}
% \label{fig:synthetic_loss_r34+}
% }
% \subfigure[]{
% \input{figs_tikz/synthetic_test_loss_a.tex}
% \label{fig:synthetic_loss_a}
% }

\begin{minipage}[t]{0.3\linewidth}
\strut\vspace*{-\baselineskip}\newline
\subfigure[Task loss for different $r_+^{(3,4)}$.]{
\input{figs_tikz/synthetic_test_loss_r34+.tex}
\label{fig:synthetic_loss_r34+}
}
\end{minipage}
\begin{minipage}[t]{0.3\linewidth}
\strut\vspace*{-\baselineskip}\newline
\subfigure[Task loss for different $a$.]{
\input{figs_tikz/synthetic_test_loss_a.tex}
\label{fig:synthetic_loss_a}
}
\end{minipage}
\begin{minipage}[t]{0.3\linewidth}
\strut\vspace*{-\baselineskip}\newline
\subfigure{
\input{figs_tikz/legend_approaches_vert.tex}
}
\end{minipage}

\caption{Simulation result with synthetic data.
% : overall task loss $\mathcal{L}_\text{total}$ under different $r_+^{(3,4)}$ (left) and different $a$ (right). 
The task losses for task-agnostic coding are too large and have to be put in a separate figure in Sec. \ref{subsec:simulation_task_ag}.}
\label{fig:synthetic_evaluation}
\end{figure}

==> figs_tex/old_2/synthetic_evaluation_appen.tex <==
\begin{figure}[t]
\centering

% \input{figs_tikz/legend_approaches.tex}
% \input{figs_tikz/legend_approaches_appen.tex}

\begin{minipage}[t]{0.3\linewidth}
\strut\vspace*{-\baselineskip}\newline
\subfigure[Task loss for different $r_+^{(3,4)}$.]{
\input{figs_tikz/synthetic_test_loss_r34+_appen.tex}
\label{fig:synthetic_loss_r34+_appen}
}
\end{minipage}
\begin{minipage}[t]{0.3\linewidth}
\strut\vspace*{-\baselineskip}\newline
\subfigure[Task loss for different $a$.]{
\input{figs_tikz/synthetic_test_loss_a_appen.tex}
\label{fig:synthetic_loss_a_appen}
}
\end{minipage}
\begin{minipage}[t]{0.3\linewidth}
\strut\vspace*{-\baselineskip}\newline
\subfigure{
\input{figs_tikz/legend_approaches_appen_vert.tex}
}
\end{minipage}

\caption{
Simulation result with synthetic data of task-agnostic coding approach.
% : overall task loss $\mathcal{L}_\text{total}$ under different $r_+^{(3,4)}$ (left) and different $a$ (right). 
}
\label{fig:synthetic_evaluation_appen}
\end{figure}

==> figs_tikz/old/legend_cube.tex <==
\begin{tikzpicture}[state/.style = {shape=rectangle,thick,draw,minimum width=+1.7ex,minimum height=+1.7ex,inner sep=+.1pt}]
% note that \tiny gets inherited from above
\matrix[column sep=1ex]{
\path (0,0.5em) node[state,fill=yellow, fill opacity=0.5,label=right:Node 1]{};\\
\path (0,0.5em) node[state,fill=cyan, fill opacity=0.5, label=right:Node 2]{};\\
\path (0,0.5em) node[state,fill=green, fill opacity=0.2, label=right:Node 3]{};\\
\path (0,0.5em) node[state,fill=red,fill opacity=0.2, label=right:Node 4]{};\\
};
\end{tikzpicture} 

==> sections/checklist.tex <==
\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{\textbf{Please see Section \ref{sec:intro}.}}
  \item Did you describe the limitations of your work?
    \answerYes{\textbf{Please see the end of the evaluation (Section \ref{sec:eval}).}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{\textbf{We do not envision any potential negative societal impacts of this work.}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{\textbf{Please see Section \ref{sec:analysis}.}}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{\textbf{Please see Section \ref{sec:analysis} and Appendix.}}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{\textbf{Please see Appendix Section \ref{subsec:training_details}.}}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{\textbf{Please see Appendix Section \ref{subsec:training_details}.}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{\textbf{Please see the citations for all three publicly-available datasets in Section \ref{sec:eval}.}}
  \item Did you mention the license of the assets?
    \answerYes{\textbf{As stated in the Appendix, the licenses for the individual assets were not given online.}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> sections/old/algorithm.tex <==
\begin{algorithm}[tb]
   \caption{Compression Co-design}
   \label{alg:codesign}
   \begin{algorithmic}[1]
       \STATE Init. encoder/decoder params. $\theta_e^i, \theta_d$ randomly
       \FOR{$t \in \{0, 1, \cdots, T-1\}$}{
           \STATE Update $\theta_d$ and $\theta_e^0$ with $-\nabla \mathcal{L}_\text{total}/ \nabla \theta_d$ and $-\nabla \mathcal{L}_\text{total}/ \nabla \theta_e^0$ by one or multiple steps

           \FOR{$i \in \{1, 2, \cdots, k\}$}{
               \STATE Update $\theta_e^i$ with $-\nabla \mathcal{L}_\text{total}/ \nabla \theta_e^i$ by one or multiple steps
            }
           \ENDFOR
       }
       \ENDFOR
       \STATE Return learned parameters $\theta_e^i, \theta_d$
    \end{algorithmic}
\end{algorithm}

==> sections/old/analysis.tex <==
Solving the given optimization problem analytically is not easy. First, similar to the single bottleneck problem \cite{DBLP:conf/rss/NakanoyaCADKP21,cheng2021data,dubois2021lossy}, if the encoder/decoder functions are allowed to be non-linear or the task loss function is non-quadratic, in general there's no analytical solution and one has to resort to machine learning approaches. Moreover, even for linear encoder and decoder functions and quadratic task loss function, multiple and heterogeneous bottlenecks, as a scenario we considering specifically, make it hard to obtain an analytical solution.


To see this, let $g_e^i(x_i; \theta_e^i) = E_i x_i, \forall i \in \{1, 2, \cdots, k\}$, where $E_i \in \reals^{r \times m}$ is the encoding matrix (corresponding to $\theta_e^i$). Similarly, let $g_e^0(\phi; \theta_e^0) = E_0 \phi$, and $g_d(\phi_0; \theta_d) = D \phi_0$, where $E_0 \in \reals^{Z \times kr}$ and $D \in \reals^{n \times Z}$, respectively. With out loss of generality, assume $E_i E_i^\top = I$.

Then we have
\begin{align}
\hat{x} 
= DE_0 
\begin{bmatrix}
E_1 x_1\\
\vdots\\
E_k x_k
\end{bmatrix}
= 
D\underbrace{
E_0 
\begin{bmatrix}
E_1 P_1\\
\vdots\\
E_k P_k
\end{bmatrix}
}_{\Phi \in \reals^{Z \times n}}
x
\end{align}
where $\Phi$ denotes the mapping from $x$ to $\phi_0$. Notice that $\Phi \Phi^\top = I$.

Suppose we only consider a quadratic task loss $\mathcal{L}_\text{task} = \E_x [\|K(x - \hat{x})\|_2^2]$, where $K \in \reals^{n \times n}$ is a task matrix. Then we have
\begin{align}
\mathcal{L}_\text{task} 
= & \E_x [\|K(x - \hat{x})\|_2^2]\\
= & \E_x [\tr(K(I-D\Phi)x x^\top (I-D\Phi)^\top)K^\top]\\
= & \tr(K(I-D\Phi)\Sigma (I-D\Phi)^\top K^\top)
\end{align}
where $\Sigma = \E_x[x x^\top]$ is the covariance matrix.

\begin{prop}
For fixed $\Phi$, the optimal $D^*$ has the form of $D^* = \Sigma \Phi^\top (\Phi \Sigma \Phi^\top)^{-1}$. And corresponding $\mathcal{L}_\text{task} = \tr(K^\top K \Sigma) - \tr(\Phi \Sigma K^\top K \Sigma \Phi^\top (\Phi \Sigma \Phi^\top)^{-1})$.
\end{prop}

\begin{proof}
\begin{align}
\frac{\nabla \mathcal{L}_\text{task}}{\nabla D} = 2 K^\top K (D \Phi \Sigma \Phi^\top - \Sigma \Phi^\top)
\end{align}
\end{proof}

Therefore, minimizing $\mathcal{L}_\text{task}$ is equivalent to maximizing $\mathcal{U}_\text{task} \triangleq \tr(\Phi \Sigma K^\top K \Sigma \Phi^\top (\Phi \Sigma \Phi^\top)^{-1})$.

If we are allowed to choose $\Phi$ arbitrarily, then according to the solution of trace-sum problem, we have $\Phi^*$ be composed of the top-$Z$ eigen-vectors of $K^\top K \Sigma$. But since sensor-edge channels are bottlenecked this may not be achievable.

\begin{prop}
Suppose the eigen-values of $K^\top K \Sigma$ are $\lambda_1, \lambda_2, \cdots, \lambda_n$, with $\lambda_1 \geq \lambda_2 \geq \cdots \geq \lambda_n$. Then $ \sum_{i=1}^r \lambda_i \leq \mathcal{U}_\text{task} \leq \sum_{i=1}^Z \lambda_i$. The equality is achievable when $Z = r$.
\end{prop}

Suppose we let $\Sigma = I$. Then $\mathcal{U}_\text{task} \triangleq \tr(\Phi K^\top K \Phi^\top)$

\begin{prop}
Suppose the eigen-values of $P_i K^\top K P_i^\top$ are $\mu_{i,1}, \mu_{i,2}, \cdots, \mu_{i,m}$, with $\mu_{i,1} \geq \mu_{i,2} \geq \cdots \geq \mu_{i,m} \geq 0$. Then $\tr(\Sigma \Phi^\top\Phi) \leq \sum_{i=1}^k \sum_{j=1}^r \mu_{i,j}$. The equality is achievable when $Z = kr$.
\end{prop}


Suppose we decompose $E_0$ into $[V_1, V_2, \cdots, V_k]$, where $V_i \in \reals^{Z \times r}$, then we have $\Phi = \sum_{i=1}^k V_i E_i P_i$. Hence
\begin{align}
\tr(\Phi K^\top K \Phi^\top) = \sum_{i=1}^k \sum_{j=1}^k \tr(V_i E_i P_i \Sigma P_j^\top  E_j^\top V_j^\top)
\end{align}
Thus the optimization problem becomes
\begin{align}
\max_{E_i} \quad & \sum_{i=1}^k \sum_{j=1}^k \tr(V_i E_i P_i \Sigma P_j^\top E_j^\top V_j^\top)\\
\text{s.t.} \quad & E_i E_i^\top = I, \quad i \in \{0, 1, \cdots, k\}\\
\quad & E_0 = [V_1, V_2, \cdots, V_k]
\end{align}
which is a non-convex optimization problem. A problem with similar structure is orthogonal trace-sum maximization (OSTM) problem defined in \cite{won2021orthogonal}. For OSTM ``we generally have to resort to iterative methods."



==> sections/old/analysis_2.tex <==
In this section, we consider a concrete problem with linear encoders, linear decoders, linear inference tasks, and mean-squared error task loss. That is, each $g_e^{i,j}$ and $g_d^i$ is a linear function of its input, each inference task has the form of
\begin{align}
\hat{y}^{(i)} = K_i \hat{x}^{(i)}, \quad \forall i \in \{3, 4\}
\end{align}
where $K_i \in \reals^{m_i \times n}$ can be viewed as the task matrix, and  

and task loss has the form of
\begin{align}
\mathcal{L}_{\text{task},i}
& = \E_x [\|y^{(i)} - \hat{y}^{(i)}\|_2^2]\\
& = \E_x [\|K^{(i)} (x^{(i)} - \hat{x}^{(i)}) \|_2^2], \quad \forall i \in \{3, 4\}
\end{align}

For simplicity of the following analysis, we let task-agnostic weight $\lambda = 0$. This assumption doesn't lose generality however.

Furthermore, we assume that $\E_x[x] = \bm{0}$ and $\E_x[xx^\top] = I$. This further implies that $\E_{x^{(1)}}[x^{(1)} x^{(1)\top}] = I$ and $\E_{x^{(2)}}[x^{(2)} x^{(2)\top}] = I$. This doesn't lose generality, because otherwise we can find one-to-one linear mappings: $x \leftrightarrow \tilde{x} \in \reals^{\tilde{n}}$, $x^{(1)} \leftrightarrow \tilde{x}^{(1)} \in \reals^{\tilde{a}}$, $x^{(2)} \leftrightarrow \tilde{x}^{(2)} \in \reals^{\tilde{b}}$, such that $\E_{\tilde{x}}[\tilde{x}] = \bm{0}$, $\E_{\tilde{x}}[\tilde{x}{\tilde{x}}^\top] = I$, and $\tilde{x}^{(1)}$ and $\tilde{x}^{(2)}$ are composed of $\tilde{a}$ and $\tilde{b}$ different dimensions of $\tilde{x}$, respectively.

For observations $x^{(1)}$ and $x^{(2)}$, we say they are 1) the same if $x^{(1)} = x^{(2)}$, i.e., $a = b = n$; 2) independent if $n = a+b$; 3) partially correlated if they are neither the same nor independent. 

For task matrix $K_i$, $\forall i \in \{3, 4\}$, suppose the eigen-values of $K_i^\top K_i$ in descending order are $\mu^{(i)}_{1}, \mu^{(i)}_{2}, \cdots, \mu^{(i)}_{n}$ and the corresponding normalized eigen-vectors are $e^{(i)}_{1}, e^{(i)}_{2}, \cdots, e^{(i)}_{n}$. We say $K_3$ and $K_4$ are 1) the same if $K_3^\top K_3 = K_4^\top K_4$; 2) independent if for any $j, j' \in \{1, 2, \cdot, n\}$, either $\mu^{(3)}_{j}\mu^{(4)}_{j'} = 0$ or $<e^{(3)}_{j}, e^{(4)}_{j'}> = 0$; 3) partially correlated if they are neither the same nor independent. In this case, we assume $K_3$ and $K_4$ has $c \leq n$ and $d \leq n$ non-zero rows respectively. Assume the $\max{c,d} \leq n \leq c + d$. Without loss of generality, we let the non-zero rows of $K_3$ corresponds to $[x_{s_1}, x_{s_2}, \cdots, x_{s_{n-d}}, x_{s_{2n-c-d+1}}, \cdots, x_{s_n}]$, the non-zero rows of $K_4$ corresponds to $[x_{s_{n-d+1}}, x_{s_{n-d+2}}, \cdots, x_{s_n}]$. Here $s_1:s_n$ is a permutation of $1:n$. That is, $x_{s_{n-d}}$ and $x_{s_{n-d+1}:s_{2n-c-d}}$ are node 1 and node 2's exclusive non-zero rows, and $x_{s_{2n-c-d+1}:s_n}$ are their mutual non-zero rows.  



Notice that when $\hat{x}^{(i)} \equiv \bm{0}, \forall i \in\{3,4\}$, we have $\mathcal{L}_{\text{task},i} = \sum_{j=1}^n \mu^{(i)}_{j}$, which is the largest task loss for node $i$ when there's no information about $x$. For convenience of the following analysis, we define $\mathcal{U}_{\text{task},i} = \sum_{j=1}^n \mu^{(i)}_{j} - \mathcal{L}_{\text{task},i}$, and $\mathcal{U}_{\text{total}} = \sum_{i=3,4} \mathcal{U}_{\text{task},i}$.

\input{figs_tex/example.tex}

Consider the vector space formulated by $e^{(3)}_{1}, e^{(3)}_{2}, \cdots, e^{(3)}_{2Z}$ and $e^{(4)}_{1}, e^{(4)}_{2}, \cdots, e^{(4)}_{2Z}$. Use $r$ to denote its rank.

\begin{thm}
$\sum_{i=3,4}\sum_{j=1}^{2Z} \mu^{(i)}_{j}$ is achievable only if $r \leq 3Z$ and the intersection of the vector space formulated by $e^{(3)\top}_{1}x, e^{(3)\top}_{2}x, \cdots, e^{(3)\top}_{2Z}x$ and the vector space formulated by $x^{(1)}$ has rank at least $Z$, and same for node 4 and node 2.
\end{thm}

%%%%%%%%%%%%
%TABLE
%%%%%%%%%%%%

\begin{table*}[t]
\caption{Optimal solution $\mathcal{U}_{\text{total}}$ for different dependencies between $x_1$ and $x_2$, and between $K_3$ and $K_4$.}
\label{tab:solution_dependency}
\vskip 0.15in
\begin{center}
\resizebox{2\columnwidth}{!}{
\begin{tabular}{l|cccr}
\toprule
Tasks $\setminus$ Observations & Same ($n=a=b$) & Independent & Correlated\\
\midrule
Same ($n=c=d$) &  $\sum_{i=3,4}\sum_{j=1}^{2Z} \mu^{(i)}_{j}$ & ? &  $\sum_{i=3,4}\sum_{j=1}^{2Z} \mu^{(i)}_{j}$ achievable when $n \leq Z + \min\{a, b\}$ \\
Independent & Determined by Algorithm \ref{alg:ind_tasks} & ? & ?  \\
Correlated &  $\sum_{i=3,4}\sum_{j=1}^{2Z} \mu^{(i)}_{j}$ achievable when $n \leq 3Z$ &  ? &  $\sum_{i=3,4}\sum_{j=1}^{2Z} \mu^{(i)}_{j}$ achievable when i) $2Z \leq r \leq 3Z + \min\{a, b\} - n$, OR\\
& & & ii) $\{s_1, \cdots, s_{n-d}, s_{2n-c-d+1}, \cdots, s_n\} \subseteq \{1, \cdots, n-b, 2n-a-b+1, \cdots, n\}$,\\
& & & $\{ s_{n-d+1}, \cdots, s_n\} \subseteq \{n-b+1, \cdots, n\}$ and $n \leq 3Z$\\
\bottomrule
\end{tabular}
}
\end{center}
\vskip -0.1in
\end{table*}

Depending on the dependencies between observations $x^{(1)}$ and $x^{(2)}$ and between task matrix $K_3$ and $K_4$, the corresponding optimal solution can vary. Jointly there are  $3 \times 3 = 9$ cases to consider, as shown in Table \ref{tab:solution_dependency}. For the four cases on the upper left corner, we determine the corresponding optimal solutions through conventional PCA and network coding technique; for the three cases on the lower right corner, the corresponding optimal solutions remains unknown analytically and we in general has to resort to machine learning approaches, which we will defer to the next section; and for the three cases on the diagonal that runs from upper right to lower left, we present the corresponding optimal solutions over some regions of the considered parameter space.

We first start with some basic common analysis that holds for all the cases.

\textbf{Upper bound for Optimal $\mathcal{U}^*_{\text{total}}$.} Notice node 3 receives $2Z$ vectors about $x$ from node 1 and node 6, and when these dimensions are
\begin{align}
e^{(3)\top}_{1} x, e^{(3)\top}_{2} x, \cdots, e^{(3)\top}_{2Z} x
\end{align}
the following reconstructed $\hat{x}_3$:
\begin{align}
\hat{x}^{(3)} = \sum_j e^{(3)}_{j} e^{(3)\top}_{j} x
\end{align}
maximizes $\mathcal{U}_{\text{task},3}$:
\begin{align}
\mathcal{U}_{\text{task},3} = \sum_{j=1}^{2Z} \mu^{(3)}_{j}
\end{align}
The result still holds if we replace node 3 by node 4. But in some cases such $\mathcal{U}_{\text{task},3}$ and $\mathcal{U}_{\text{task},4}$ are not achievable. Therefore, we have
\begin{align}
\mathcal{U}^*_{\text{total}} \leq \sum_{i=3,4} \sum_{j=1}^{2Z} \mu^{(i)}_{j}
\end{align}

We next perform analysis on a case-by-case basis.

\subsection{Same tasks, same observations}
$\mathcal{U}^*_{\text{total}} = \sum_{i=3,4} \sum_{j=1}^{2Z} \mu_{i,j}$ is achievable. In this case, $\mu^{(3)}_{k} = \mu^{(4)}_{k}$ and $e^{(3)}_{k} = e^{(4)}_{k}$, for any $k$. So we simply let $\phi^{(6,3)} = \phi^{(6,4)} = [e^{(3)\top}_{1} x, e^{(3)\top}_{2} x, \cdots, e^{(3)\top}_{Z} x]^\top$ and $\phi^{(1,3)} = \phi^{(2,4)} = [e^{(3)\top}_{Z+1} x, e^{(3)\top}_{Z+2} x, \cdots, e^{(3)\top}_{2Z} x]^\top$.

\subsection{Independent tasks, same observations}

$\mathcal{U}^*_{\text{total}}$ is determined by Algorithm \ref{alg:ind_tasks}, where we select the top-$3Z$ eigen-values among $\mu_{i,k}$, $\forall i \in \{3, 4\}, k \in \{1,2, \cdots, n\}$, where the number of selected eigen-values for task $i$ ($\forall i \in \{3, 4\}$) is no more than $2Z$. We then let $[\phi^{(6,3)\top}, \phi^{(1,3)\top} ]^\top$ be the associated eigen-vectors times $x$ for task 3, and similarly for task 4.

Such approach is optimal because, we know for any dimension of $\phi^{(5,6)}$, denoted by $\xi^\top x \in \reals$ where $\xi \in \reals^n$, we can decompose $\xi$ into $\alpha \xi_1 + \beta \xi_2$ such that $\xi^\top (K_3^\top K_3 + K_4^\top K_4)\xi = \alpha^2 \xi_1^\top K_3^\top K_3 \xi_1 + \beta^2 \xi_2^\top K_4^\top K_4 \xi_2$, with $\alpha^2 + \beta^2 = 1$. And for any dimension of $\phi^{(1,3)}$, denoted by $\xi^\top x \in \reals$ where $\xi \in \reals^n$, only has contribution to $\xi^\top K_3^\top K_3 \xi$. So overall the sum of coefficients is $3Z$, and for each task the sum of the associated coefficients is no more than $2Z$.

\begin{algorithm}[tb]
   \caption{Optimal $\mathcal{U}^*_{\text{total}}$ for independent tasks, same observations}
   \label{alg:ind_tasks}
   \begin{algorithmic}[1]
       \STATE Input $\mu^{(i)}_{k}$, $\forall i \in \{3, 4\}, k \in \{1,2, \cdots, n\}$
       \STATE $\mathcal{U} = 0$
       \STATE $count = 0$, $count_i$ = 0, $\forall i \in \{3, 4\}$
       \STATE Sort $\mu^{(i)}_{k}$ in the descending order
       \FOR{$\mu^{(i)}_{k}$ in the descending order}{
           \IF{$count_i == 2Z$}{
                \STATE continue
           }
           \ENDIF
           \STATE $\mathcal{U} \mathrel{+}= \mu^{(i)}_{k}$
           \STATE $count \mathrel{+}= 1$, $count_i \mathrel{+}= 1$
           \IF{$count == 3Z$}{
                \STATE break
           }
           \ENDIF
       }
       \ENDFOR
       \STATE Return $\mathcal{U}$
    \end{algorithmic}
\end{algorithm}

\subsection{Same tasks, independent observations}
TBD

\subsection{Independent tasks, independent observations}
TBD

\subsection{Same tasks, correlated observations}

For correlated observations, since at least one of the node 1 and node 2 do not possess the full data, we may not be able to achieve the same utility as in the ``same tasks, same observations" case.

However, we find a sufficient condition with respect to $n, a, b, Z$ to achieve the same utility.

\begin{thm}
If $n \leq Z + \min\{a, b\}$, $\mathcal{U}^*_{\text{total}} = \sum_{i=3,4} \sum_{j=1}^{2Z} \mu^{(i)}_{j}$ is achievable.
\end{thm}

\input{figs_tex/explanation.tex}

\begin{proof}
To achieve $\mathcal{U}^*_{\text{total}} = \sum_{i=3,4} \sum_{j=1}^{2Z} \mu^{(i)}_{j}$, both node $3$ and node $4$ should be able to correctly decode $e^{(3)\top}_{1} x, e^{(3)\top}_{2} x, \cdots, e^{(3)\top}_{2Z} x$. Notice that $e^{(3)}_{1}, e^{(3)}_{2}, \cdots, e^{(3)}_{2Z}$ are orthogonal.

We let
\begin{align}
\Xi =
\begin{bmatrix}
\xi^\top_{1}\\
\xi^\top_{2}\\
\vdots\\
\xi^\top_{2Z}
\end{bmatrix}
= 
\begin{bmatrix}
e^{(3)\top}_{1}\\
e^{(3)\top}_{2}\\
\vdots\\
e^{(3)\top}_{2Z}
\end{bmatrix}
\in \reals^{2Z \times n}
\end{align}
whose row vectors are composed of $e^{(3)}_{1}, e^{(3)}_{2}, \cdots, e^{(3)}_{2Z}$. We next perform Gauss-Jordan elimination over $\Xi$, which transforms $\Xi$ in its reduced row echelon form, which has the following two properties:
\begin{itemize}
\item The leading coefficient of a nonzero row is always strictly to the right of the leading coefficient of the row above it, and is always 1 (called a leading 1);
\item Each column containing a leading 1 has zeros in all its other entries. 
\end{itemize}

The left part of $\Xi$ is not necessarily an identity matrix. suppose only $\xi_{1:n-b'}$ have non-zero elements for the first $n-b$ columns, where $b' \geq b$; and only $\xi_{n-b'+1:2n-b'-a'}$ have non-zero elements for the next $n-a$ columns in the remaining row vectors, where $a' \geq a$. Then $\xi_{2n-b'-a':2Z}$ have only zero elements for the first $2n-a-b$ columns.

Here $\xi_{1:n-b'}$ may have non-zero elements for the columns corresponding to $x_{n-b+1:2n-a-b}$. But the number of such columns, denoted by $c$, is at most $\min \{n-b', a' - a\}$. Without loss of generality, assume the $\xi_{1:c}$   

We then do Gauss-Jordan elimination again for $\xi_{1:n-b'}$ to make the columns corresponding to $x_{n-b+1:2n-a-b}$ has the properties mentioned above. Note that now the first $n-b$ columns of $\xi_{1:n-b'}$ doesn't have the properties anymore. Suppose the $\xi_{1:c'}$ have non-zero elements for the the columns corresponding to $x_{n-b+1:2n-a-b}$, where $c' < c$. Then our encoding approach is:

1) Middle link sends $\xi_{1}^\top x, \cdots, \xi_{c'}^\top x$ by consulting both node 1 and node 2;

2) node 1 and node 2 remain $Z-c'$ to send on the middle link. Node 1 choose $\xi_{c'+1}^\top x, \xi_{c'+2}^\top x, \cdots, \xi_{n-b'}^\top x$ and $\xi_{2n-a'-b'+1}^\top x, \cdots, \xi_{Z+n-a'}^\top x$. Node 2 choose $\xi_{n-b'+1}^\top x, \xi_{n-b'+2}^\top x, \cdots, \xi_{2n-a'-b'}^\top x$ and $\xi_{Z+n-a'+1}^\top x, \cdots, \xi_{2Z-c'}^\top x$. Middle link do a element-wise sum for these $Z-c'$ dimensions.

3) For the private link $(1,3)$, node 1 sends $\xi_{c'+1}^\top x, \xi_{c'+2}^\top x, \cdots, \xi_{n-b'}^\top x$ and $\xi_{2Z-c'+1}^\top x, \cdots, \xi_{2Z}^\top x$. For the private link $(2,4)$, node 2 sends $\xi_{n-b'+1}^\top x, \xi_{n-b'+2}^\top x, \cdots, \xi_{2n-a'-b'}^\top x$ and $\xi_{2Z-c'+1}^\top x, \cdots, \xi_{2Z}^\top x$.

\end{proof} 

\subsection{Correlated tasks, same observations}

% (Keep or not?) If the contributions of $x_{s_{2n-c-d+1}:s_n}$ are exactly the same to both tasks. We find a sufficient condition with respect to $n, c, d, Z$ to achieve the same utility. 

% \begin{thm}
% If $n \leq Z + \min\{c, d\}$, $\mathcal{U}^*_{\text{total}} = \sum_{i=3,4} \sum_{j=1}^{2Z} \mu^{(i)}_{j}$ is achievable.
% \end{thm}

We find a sufficient condition with respect to $n, Z$ to achieve the same utility.

\begin{thm}
If $n \leq 3Z$, $\mathcal{U}^*_{\text{total}} = \sum_{i=3,4} \sum_{j=1}^{2Z} \mu^{(i)}_{j}$ is achievable.
\end{thm}

\begin{proof}
Consider $e^{(3)}_{1}, e^{(3)}_{2}, \cdots, e^{(3)}_{2Z}$ and $e^{(4)}_{1}, e^{(4)}_{2}, \cdots, e^{(4)}_{2Z}$. They together form a vector space of rank at most $n \leq 3Z$. So the intersection of two vector space is at least $4Z - n \geq Z$. Therefore, the middle link sends $Z$ independent vectors in the intersection, and each private link sends the rest $Z$ vectors in their own vector space.
\end{proof}

\subsection{Correlated tasks, correlated observations}

\begin{thm}
Suppose $\{s_1, \cdots, s_{n-d}, s_{2n-c-d+1}, \cdots, s_n\} \subseteq \{1, \cdots, n-b, 2n-a-b+1, \cdots, n\}$, and $\{ s_{n-d+1}, \cdots, s_n\} \subseteq \{n-b+1, \cdots, n\}$. That is, the task for node 3 is only dependent on the observation of node 1, and same for node 4 and node 2. Then if $n \leq 3Z$, $\mathcal{U}^*_{\text{total}} = \sum_{i=3,4} \sum_{j=1}^{2Z} \mu^{(i)}_{j}$ is achievable.
\end{thm}

\begin{proof}
Same as above.
\end{proof}

\begin{thm}
Consider the vector space formulated by $e^{(3)}_{1}, e^{(3)}_{2}, \cdots, e^{(3)}_{2Z}$ and $e^{(4)}_{1}, e^{(4)}_{2}, \cdots, e^{(4)}_{2Z}$. If its rank $r$ satisfies $ 2Z \leq r \leq 3Z + \min\{a, b\} - n$,  $\mathcal{U}^*_{\text{total}} = \sum_{i=3,4} \sum_{j=1}^{2Z} \mu^{(i)}_{j}$ is achievable.
\end{thm}

\begin{proof}
$e^{(3)}_{1}, e^{(3)}_{2}, \cdots, e^{(3)}_{2Z}$ and $e^{(4)}_{1}, e^{(4)}_{2}, \cdots, e^{(4)}_{2Z}$ have $4Z-r \geq Z$ common vectors, and $r-2Z \leq Z$ exclusive vectors. We first send $r-2Z$ exclusive vectors on the private links. The private links have capacity $3Z -r$ remaining.

We hope to broadcast the remaining $4Z - r$ vectors using the residual network.
Note that $n-a, n-b \leq 3Z -r$. This is doable through the similar Gauss-Jordan elimination.
\end{proof}

% We find a sufficient condition with respect to $n, a, b, Z$ to achieve the same utility.

% \begin{thm}
% If $n \leq 3Z$, $\mathcal{U}^*_{\text{total}} = \sum_{i=3,4} \sum_{j=1}^{2Z} \mu^{(i)}_{j}$ is achievable.
% \end{thm}







==> sections/old/analysis_3.tex <==
We first show that making the assumption of $\text{rank}(\Psi) = n$ doesn't make the considered problem lose generality. 

\begin{theorem}
For any $n, \Psi, a, b, Z, K^{(3)}, K^{(4)}$, we can find $\tilde{n}, \tilde{\Psi}, \tilde{a}, \tilde{b}, Z, \tilde{K}^{(3)}, \tilde{K}^{(4)}$ such that the task-aware network coding problem under these two sets of parameters are equivalent, and $\text{rank}(\tilde{\Psi}) = \tilde{n}$. That is, $\mathcal{L}_\text{total}(n, \Psi, a, b, Z, K^{(3)}, K^{(4)}) = \mathcal{L}_\text{total}(\tilde{n}, I, \tilde{a}, \tilde{b}, Z, \tilde{K}^{(3)}, \tilde{K}^{(4)})$.  
\end{theorem}

\begin{proof}
Assume the top-$\tilde{n}$ eigen-values of $\Psi$ are greater than zero, where $\tilde{n} \leq n$. We use $\lambda_1, \cdots, \lambda_{\tilde{n}}$ to denote these eigen-values and $q_1, \cdots, q_{\tilde{n}}$ to denote the corresponding normalized eigen-vectors. Moreover, we let $\Lambda = \diag\{\lambda_1, \cdots, \lambda_{\tilde{n}}\} \in \reals^{\tilde{n} \times \tilde{n}}$ and $Q = [q_1, \cdots, q_{\tilde{n}}] \in \reals^{n \times \tilde{n}}$.

Consider $\tilde{x} = \Lambda^{-\frac{1}{2}} Q^\top x \in \reals^{\tilde{n}}$. We have $\E [\tilde{x}\tilde{x}^\top] = \Lambda^{-\frac{1}{2}} Q^\top \Psi Q \Lambda^{-\frac{1}{2}} = I$. And we also have $x = Q \Lambda^{\frac{1}{2}} \tilde{x}$. For simplicity we let $L = (Q \Lambda^{\frac{1}{2}})^\top$ and $l_i$ to denote the $i$-th column vector of $L$. Let $L_1 = [l_1, \cdots, l_{a}] \in \reals^{\tilde{n} \times (n-a)}$ and $L_2 = [l_{n-b+1}, \cdots, l_n] \in \reals^{\tilde{n} \times (n-b)}$. Let $\tilde{a} = \dm(\sn(L_1))$ and $\tilde{b} = \dm(\sn(L_2))$, where $\sn(\cdot)$ is the column span of a matrix. Then we have $\dm(\sn(L_1) \cap \sn(L_2)) = \tilde{a} + \tilde{b} - \tilde{n}$, and we can find $v_{\tilde{n}-\tilde{b}+1}, \cdots, v_{\tilde{a}}$ that form an orthogonal basis of $\sn(L_1) \cap \sn(L_2)$. Furthermore, we can also find $v_1, \cdots, v_{\tilde{n}-\tilde{b}}$ and $v_{\tilde{a}+1}, \cdots, v_{\tilde{n}}$ such that together with $v_{\tilde{n}-\tilde{b}+1}, \cdots, v_{\tilde{a}}$ they form an orthogonal basis of $\sn(L_1)$ and $\sn(L_2)$, respectively. Therefore, we let $\tilde{x}' = V^\top \tilde{x}$ where $V = [v_1, \cdots, v_{\tilde{n}}] \in \reals^{\tilde{n} \times \tilde{n}}$. Since $V^\top V = I$, we also have $\E [\tilde{x}'\tilde{x}'^\top] = I$. The transformations between $x$ and $\tilde{x}'$  are $x = Q \Lambda^{-\frac{1}{2}} V \tilde{x}'$ and $\tilde{x}' = V^\top \Lambda^{-\frac{1}{2}} Q^\top x$ (Note that there are more than one transformation from $x$ to $\tilde{x}'$ if $\tilde{n} < n$). And from the construction process we have $\forall i \in \{1, \cdots, a\}$, $x_i$ can be expressed as a linear combination of $\tilde{x}'_1, \cdots, \tilde{x}'_{\tilde{a}}$; $\forall i \in \{n-b+1, \cdots, n\}$, $x_i$ can be expressed as a linear combination of $\tilde{x}'_{\tilde{n}-\tilde{b}+1}, \cdots, \tilde{x}'_{\tilde{n}}$. The same conclusion still holds if we switch $n, a, b, x$ and $\tilde{n}, \tilde{a}, \tilde{b}, \tilde{x}'$.

$\forall i \in \{3, 4\}$, we define $\tilde{K}^{(i)} = K^{(i)} Q \Lambda^{-\frac{1}{2}} V \in \reals^{m_i \times \tilde{n}}$. Therefore, $\tilde{K}^{(i)} \tilde{x}' = K^{(i)} x$. Then we claim that the task-aware network coding problem under parameters $n, \Psi, a, b, Z, K^{(3)}, K^{(4)}$ and $\tilde{n}, I, \tilde{a}, \tilde{b}, Z, \tilde{K}^{(3)}, \tilde{K}^{(4)}$ are equivalent. 
To show this, consider an valid solution $\{\tilde{E}^{(i,j)}, \tilde{D}^{(i)}\}$ for the task-aware network coding problem under parameters $\tilde{n}, I, \tilde{a}, \tilde{b}, Z, \tilde{K}^{(3)}, \tilde{K}^{(4)}$. We can manipulate each $E^{(i,j)}$ to make $\phi^{(i,j)} = \tilde{\phi}^{(i,j)}$, $\forall (i, j) \in \mathcal{E}$. For example, we can let $E^{(1,3)} = \tilde{E}^{(1,3)} M$ where $M \in \reals^{\tilde{a} \times a}$ is a linear transformation from $x_1, \cdots, x_a$ to $\tilde{x}'_1, \cdots, \tilde{x}'_{\tilde{a}}$. Moreover, we also let $D^{(i)} = Q \Lambda^{-\frac{1}{2}} V \tilde{D}^{(i)}$, $\forall i \in \{3, 4\}$. In this way an valid solution $\{\tilde{E}^{(i,j)}, \tilde{D}^{(i)}\}$ is transformed to an valid solution $\{E^{(i,j)}, D^{(i)}\}$. The reverse is also true. Hence the task-aware network coding problem under parameters $n, \Psi, a, b, Z, K^{(3)}, K^{(4)}$ and $\tilde{n}, I, \tilde{a}, \tilde{b}, Z, \tilde{K}^{(3)}, \tilde{K}^{(4)}$ are equivalent, and $\mathcal{L}_\text{total}(n, \Psi, a, b, Z, K^{(3)}, K^{(4)}) = \mathcal{L}_\text{total}(\tilde{n}, I, \tilde{a}, \tilde{b}, Z, \tilde{K}^{(3)}, \tilde{K}^{(4)})$.
\end{proof}

Therefore, in the rest of the analysis, we simply consider $\Psi = I$. Furthermore, we assume $Z \leq n$, or else the network is not bottlenecked. 

% For observations $x^{(1)}$ and $x^{(2)}$, we say they are 1) the same if $x^{(1)} = x^{(2)}$, i.e., $a = b = n$; 2) independent if $n = a+b$; 3) partially correlated if they are neither the same nor independent. 

For task matrix $K^{(i)}$, $\forall i \in \{3, 4\}$, we define Gram matrix $S^{(i)} = K^{(i)\top} K^{(i)} \in \reals^{n \times n}$. Moreover, let the eigen-values of $S^{(i)}$ in descending order be $\mu^{(i)}_{1}, \mu^{(i)}_{2}, \cdots, \mu^{(i)}_{n}$ and the corresponding normalized eigen-vectors be $u^{(i)}_{1}, u^{(i)}_{2}, \cdots, u^{(i)}_{n}$. Since node 3 receives $[\phi^{(1,3)\top}, \phi^{(6,3)\top}]^\top$ which has $2Z$ dimensions, according PCA (as we have discussed in Section \ref{subsec:preliminary_pca}), we have $\mathcal{L}^{(3)} \geq \sum_{j={2Z+1}}^n \mu^{(3)}_{j}$ (note if $2Z+1 > n$, the right-hand side is simply 0). Similarly, $\mathcal{L}^{(4)} \geq \sum_{j={2Z+1}}^n \mu^{(4)}_{j}$. Therefore, $\mathcal{L}_{\text{total}} \geq \mathcal{L}_{\text{total,lb}}$ where $\mathcal{L}_{\text{total,lb}} = \sum_{i=3,4} \sum_{j={2Z+1}}^n \mu^{(3)}_{j}$.


% We say $K_3$ and $K_4$ are 1) the same if $K_3^\top K_3 = K_4^\top K_4$; 2) independent if for any $j, j' \in \{1, 2, \cdot, n\}$, either $\mu^{(3)}_{j}\mu^{(4)}_{j'} = 0$ or $<e^{(3)}_{j}, e^{(4)}_{j'}> = 0$; 3) partially correlated if they are neither the same nor independent.

Ideally, we want to find a solution such that $\mathcal{L}^*_{\text{total}} = \mathcal{L}_{\text{total,lb}}$, but it may not be always achievable. Hence in the rest of this section, we focus on exploring the necessary conditions and sufficient conditions for $\mathcal{L}^*_{\text{total}} = \mathcal{L}_{\text{total,lb}}$.

$\forall i \in \{3, 4\}$, we define 
$$U^{(i)} = [u^{(i)}_{1}, u^{(i)}_{2}, \cdots, u^{(i)}_{\min\{2Z,n\}}] \in \reals^{n \times \min\{2Z,n\}},$$
where the column vectors of $U^{(i)}$ are the top-$\min\{2Z,n\}$ eigen-vectors of $\Phi^{(i)}$. And we let $U^{(1)} \in \reals^{n \times a}$ and $U^{(2)} \in \reals^{n \times b}$ be composed of the first $a$ and last $b$ columns of an $n \times n$ identity matrix.  Moreover, we also let $r_+^{(3,4)} = \dm(\sn\{[U^{(3)}, U^{(4)}]\})$, $r_-^{(3,4)} = \dm(\sn\{U^{(3)}\} \cap \sn\{U^{(4)}\}\})$, $r_-^{(1,3)} = \dm(\sn\{U^{(1)}\} \cap \sn\{U^{(3)}\}\})$, and $r_-^{(2,4)} = \dm(\sn\{U^{(2)}\} \cap \sn\{U^{(4)}\}\})$. Notice that $r_+^{(3,4)} + r_-^{(3,4)} = 2 \min\{2Z,n\}$.

We can find orthogonal basis $v_1, \cdots, v_{r_+^{(3,4)}} \in \reals^n$ for $\sn\{[U^{(3)}, U^{(4)}]\}$ such that the $v_1, \cdots, v_{\min\{2Z, n\}}$ and $v_{r_+^{(3,4)}-\min\{2Z, n\}+1}, \cdots, v_{r_+^{(3,4)}}$ are basis for $\sn\{U^{(3)}\}$ and $\sn\{U^{(4)}\}$ respectively, and $v_{r_+^{(3,4)}-\min\{2Z, n\}+1}, \cdots, v_{\min\{2Z, n\}}$ is a basis for $\sn\{U^{(3)}\} \cap \sn\{U^{(4)}\}$.


% \begin{align} 
% r = \dm(\sn\{
% & \\
% & e^{(4)}_{1}, e^{(4)}_{2}, \cdots, e^{(4)}_{\min\{2Z,n\}}
% \}),
% \end{align}
% which is the dimension of the span of the top-$\min\{2Z,n\}$ eigen-vectors of $\Phi^{(3)}$ and $\Phi^{(4)}$.

\subsection{Necessary condition}

The following Theorem \ref{thm:nc} provides a necessary condition to achieve $\mathcal{L}_{\text{total,lb}}$ under a mild assumption.

\begin{theorem} \label{thm:nc}
Assume $2Z \geq n$ or $\mu^{(i)}_{2Z} > \mu^{(i)}_{2Z+1}$, $\forall i \in \{3, 4\}$. Then $\mathcal{L}_{\text{total,lb}}$ is achievable only when $r_+^{(3,4)} \leq 3Z$, $r_-^{(1,3)} \geq \min\{Z,n-Z\}$ and $r_-^{(2,4)} \geq \min\{Z,n-Z\}$.
\end{theorem}

\begin{proof}
If $2Z \geq n$ or $\mu^{(i)}_{2Z} > \mu^{(i)}_{2Z+1}$, $\mathcal{L}_{\text{total,lb}}$ is achievable if and only if node 3 and node 4 can decode the column vectors of $U^{(3)}$ and $U^{(4)}$, i.e., $\sn\{U^{(3)}\} \subset \sn\{[\Phi^{(1,3)}, \Phi^{(6,3)}]\}$ and $\sn\{U^{(4)}\} \subset \sn\{[\Phi^{(2,4)}, \Phi^{(6,4)}]\}$.

Notice that $\{(1, 3), (2, 4), (5,6)\}$ is the cut set between node 1, 2, 5 and node 3, 4, 6, and it can transmits $3Z$ dimensions at most. Thus when $r_+^{(3,4)} > 3Z$ it is impossible to transmit the column vectors of $U^{(3)}$ and $U^{(4)}$ simultaneously from node 1, 2, 5 to node 3, 4, 6 with linear encoding and decoding. So $\mathcal{L}_{\text{total,lb}}$ is not achievable.

Moreover, notice that path $2 \rightarrow 5 \rightarrow 6 \rightarrow 3$ is the only path from node 2 to node 3, which can transmits $Z$ dimensions at most. Hence if $r_-^{(1,3)} < \min\{Z,n-Z\}$, we have $r_-^{(1,3)} + Z < \min\{2Z,n\}$, that is, node 1 and node 2 together are not able to transmit the column vectors of $U^{(3)}$ to node 3. So $\mathcal{L}_{\text{total,lb}}$ is not achievable. Similarly, $\mathcal{L}_{\text{total,lb}}$ is not achievable when $r_-^{(2,3)} < \min\{Z,n-Z\}$.

Therefore the theorem is proved. 
\end{proof}

\input{figs_tex/example.tex}

To show the conditions in Theorem \ref{thm:nc} are only necessary but not sufficient, we present two examples in Fig. \ref{fig:exp}, where we have $n=3$, $Z = 1$, $a = b = 2$, so $x^{(1)} = [x_1, x_2]^\top$ and $x^{(2)} = [x_2, x_3]^\top$. And we also assume $\mu^{(i)}_{2} > \mu^{(i)}_{3}$, $\forall i \in \{3, 4\}$. To achieve $\mathcal{L}_{\text{total,lb}}$, we must have $\sn\{[\Phi^{(1,3)}, \Phi^{(6,3)}]\} = \sn\{U^{(3)}\}$ and $\sn\{[\Phi^{(2,4)}, \Phi^{(6,4)}]\} = \sn\{U^{(4)}\}$.

In Fig. \ref{fig:exp1}, we assume $u^{(3)}_{1} = u^{(4)}_{1} = [0, 1, 0]^\top$, $u^{(3)}_{2} = [0, 0, 1]^\top$ and $u^{(4)}_{2} = [1, 0, 0]^\top$. So we have $r_+^{(3,4)} = 3$ and $r_-^{(1,3)} = r_-^{(1,4)} = 1$. The conditions in Theorem \ref{thm:nc} are satisfied, but $\mathcal{L}_{\text{total,lb}}$ is not achievable. This is because, if $\Phi^{(6,3)} = \Phi^{(6,4)} = [0, \alpha, 0]^\top$ where $\alpha$ is a non-zero real number, then we must have $\Phi^{(1,3)} = [\beta, \gamma, 0]^\top$ where $\beta$ is a non-zero real number, but this is impossible because $x_1$ is not in $x^{(1)}$; If $\Phi^{(6,3)} = \Phi^{(6,4)} \neq [0, \alpha, 0]^\top$ where $\alpha$ is a non-zero real number, we cannot make $\sn\{[\Phi^{(1,3)}, \Phi^{(6,3)}]\} = \sn\{U^{(3)}\}$ and $\sn\{[\Phi^{(2,4)}, \Phi^{(6,4)}]\} = \sn\{U^{(4)}\}$ simultaneously (for example, if $\Phi^{(6,3)}$ is not on the plane $x_1 = 0$, we will not have $\sn\{[\Phi^{(1,3)}, \Phi^{(6,3)}]\} = \sn\{U^{(3)}\}$).

In Fig. \ref{fig:exp2}, we assume $u^{(3)}_{1} = u^{(4)}_{1} = \frac{1}{\sqrt{11}}[1, 1, 3]^\top$, $u^{(3)}_{2} = \frac{1}{\sqrt{66}} [4, -7, 1]^\top$ and $u^{(4)}_{2} = \frac{1}{\sqrt{66}} [-7, 4, 1]^\top$. If we let $\Phi^{(6,3)} = \Phi^{(6,4)} = [1, 3, 1]^\top$, and $\Phi^{(1,3)} = [0, 1, 1]^\top$ and $\Phi^{(2,4)} = [1, 0, 1]^\top$, we will have $\sn\{[\Phi^{(1,3)}, \Phi^{(6,3)}]\} = \sn\{U^{(3)}\}$ and $\sn\{[\Phi^{(2,4)}, \Phi^{(6,4)}]\} = \sn\{U^{(4)}\}$. Thus $\mathcal{L}_{\text{total,lb}}$ is achievable. On thing interesting to notice is even though $\Phi^{(1,3)}$ is neither $u^{(3)}_{1}$ and $u^{(3)}_{2}$ (and similarly for $\Phi^{(2,4)}$), we are still able to achieve $\mathcal{L}_{\text{total,lb}}$.

%%%%%%%%%%%%
%TABLE
%%%%%%%%%%%%

\begin{table*}[t]
\caption{Sufficient conditions to achieve $\mathcal{L}_{\text{total,lb}}$.}
\label{tab:sf}
\vskip 0.15in
\begin{center}
\begin{tabular}{C{0.15\linewidth} | C{0.2\linewidth} | C{0.55\linewidth}}
\toprule
\multirow{2}{*}{Observations} & \multicolumn{2}{c}{Tasks}\\
\cline{2-3}
 & Same ($S^{(3)} = S^{(4)}$) & Not Same\\
\midrule
Same ($a=b=n$) &  \makecell{Theorem \ref{thm:sf1}: \\ Always achievable} & Corollary \ref{cor:sf2}: $r_+^{(3,4)} \leq 3Z$ \\
\hline
Not Same & \makecell{Corollary \ref{cor:sf3}: \\ $n \leq Z + \min\{a, b\}$} & 
\makecell{
The following 1 and 2a (Theorem \ref{thm:sf2}) \textbf{or} 1 and 2b (Theorem \ref{thm:sf3})\\
1) $r_+^{(3,4)} \leq 3Z$,\\
$v_1, \cdots, v_{r_+^{(3,4)}-\min\{2Z, n\}} \in \sn\{U^{(1)}\}$,\\
and $v_{\min\{2Z, n\}+1}, \cdots, v_{r_+^{(3,4)}} \in \sn\{U^{(2)}\}$;\\ 
2a) $v_{r_+^{(3,4)}-\min\{2Z, n\}+1}, \cdots, v_{\min\{2Z, n\}} \in \sn\{U^{(1)}\} \cap \sn\{U^{(2)}\}$;\\ 
2b) $n \leq Z + \min\{a, b\}$.
}
\\
\bottomrule
\end{tabular}
\end{center}
\vskip -0.1in
\end{table*}

\subsection{Sufficient Conditions}

In this subsection we give a few sufficient conditions such that $\mathcal{L}_{\text{total,lb}}$ is achievable. A fundamental sufficient condition is $\sn\{U^{(3)}\} \subset \sn\{[\Phi^{(1,3)}, \Phi^{(6,3)}]\}$ and $\sn\{U^{(4)}\} \subset \sn\{[\Phi^{(2,4)}, \Phi^{(6,4)}]\}$. We will next give concrete sufficient conditions for the parameters $n, a, b, Z, K^{(3)}, K^{(4)}$, based on the fundamental sufficient condition, such that $\mathcal{L}_{\text{total,lb}}$ is achievable. The results in this subsection is summarized in Table \ref{tab:sf}.

The following Theorem \ref{thm:sf1} gives the simplest sufficient condition such that $\mathcal{L}_{\text{total,lb}}$ is achievable, and network coding is not needed.

\begin{theorem}\label{thm:sf1}
If $a = b = n$ and $S^{(3)} = S^{(4)}$, i.e., the observations and the tasks are the same, $\mathcal{L}_{\text{total,lb}}$ is achievable.
\end{theorem}

\begin{proof}
When $S^{(3)} = S^{(4)}$, we have $\mu^{(3)}_j = \mu^{(4)}_j$ and $u^{(3)}_j = u^{(4)}_j$, $\forall j \in \{1, 2, \cdots, n\}$. And we can find encoders that make the column vectors of $\Phi^{(6,3)} = \Phi^{(6,4)}$ and $\Phi^{(1,3)} = \Phi^{(2,4)}$ be the first $Z$ and last $Z$ column vectors of $U^{(3)}$. Therefore, $\sn\{[\Phi^{(1,3)}, \Phi^{(6,3)}]\} = \sn\{[\Phi^{(2,4)}, \Phi^{(6,4)}]\} = \sn\{U^{(3)}\} = \sn\{U^{(4)}\}$, and hence $\mathcal{L}_{\text{total,lb}}$ is achievable.
\end{proof}

\begin{theorem}\label{thm:sf2}
If 
% 1) $\{s_1, \cdots, s_{c}\} \subseteq \{1, \cdots, a\}$, and $\{ s_{n-d+1}, \cdots, s_n\} \subseteq \{n-b+1, \cdots, n\}$, i.e., $K^{(3)}$ is only related to $x^{(1)}$, and $K^{(4)}$ is only related to $x^{(2)}$, 
1) $r_+^{(3,4)} \leq 3Z$, $v_1, \cdots, v_{r_+^{(3,4)}-\min\{2Z, n\}} \in \sn\{U^{(1)}\}$, $v_{\min\{2Z, n\}+1}, \cdots, v_{r_+^{(3,4)}} \in \sn\{U^{(2)}\}$ and 2) $v_{r_+^{(3,4)}-\min\{2Z, n\}+1}, \cdots, v_{\min\{2Z, n\}} \in \sn\{U^{(1)}\} \cap \sn\{U^{(2)}\}$, 
% i.e., the exclusive base vectors for $\sn\{U^{3}\}$ and $\sn\{U^{4}\}$ are in $\sn\{U^{(1)}\}$ and $\sn\{U^{(2)}\}$, respectively, and the common base vectors for $\sn\{U^{3}\}$ and $\sn\{U^{4}\}$ are in $\sn\{U^{(1)}\} \cap \sn\{U^{(2)}\}$,
then $\mathcal{L}_{\text{total,lb}}$ is achievable.
\end{theorem}

\begin{proof}
Since $r_+^{(3,4)} \leq 3Z$, we have $r_-^{(3,4)} \geq 2\min\{2Z, n\} - 3Z$. 
We first randomly choose $Z$ vectors among $v_{r_+^{(3,4)}-\min\{2Z, n\}+1}, \cdots, v_{\min\{2Z, n\}}$ to be the column vectors of $\Phi^{(6,3)} = \Phi^{(6,4)}$. If $r_-^{(3,4)} < Z$ we allow $Z - r_-^{(3,4)}$ vectors to be redundant.
We next randomly choose another $Z$ vectors among $v_1, \cdots, v_{\min\{2Z, n\}}$ and $v_{r_+^{(3,4)}-\min\{2Z, n\}+1}, \cdots, v_{r_+^{(3,4)}}$, which have at least all the vectors not chosen for $\Phi^{(6,3)} = \Phi^{(6,4)}$ (the number of which is $\min\{2Z, n\} - \min\{Z, r_-^{(3,4)}\} \leq Z$), to be the column vectors of $\Phi^{(1,3)}$ and $\Phi^{(6,4)}$ respectively. This is possible because $v_1, \cdots, v_{r_+^{(3,4)}} \in \sn\{U^{(1)}\}$ and $v_{r_+^{(3,4)}-\min\{2Z, n\}+1}, \cdots, v_{r_+^{(3,4)}} \in \sn\{U^{(2)}\}$.
% Since $\{s_1, \cdots, s_{c}\} \subseteq \{1, \cdots, a\}$, and $\{ s_{n-d+1}, \cdots, s_n\} \subseteq \{n-b+1, \cdots, n\}$, we know that such $\Phi^{(1,3)}$ and $\Phi^{(6,4)}$ are related to $x^{(1)}$ and $x^{(2)}$ only and are hence valid.

It can be verified that $\sn\{[\Phi^{(1,3)}, \Phi^{(6,3)}]\} = \sn\{U^{(3)}\}$ and $\sn\{[\Phi^{(2,4)}, \Phi^{(6,4)}]\} = \sn\{U^{(4)}\}$, which means $\mathcal{L}_{\text{total,lb}}$ is achievable.
\end{proof}

\begin{corollary}\label{cor:sf2}
If $a =b = n$, i.e., the observations are the same, and $r_+^{(3,4)} \leq 3Z$, then $\mathcal{L}_{\text{total,lb}}$ is achievable.
\end{corollary}

\begin{theorem}\label{thm:sf3}
If 1) $r_+^{(3,4)} \leq 3Z$, $v_1, \cdots, v_{r_+^{(3,4)}-\min\{2Z, n\}} \in \sn\{U^{(1)}\}$, $v_{\min\{2Z, n\}+1}, \cdots, v_{r_+^{(3,4)}} \in \sn\{U^{(2)}\}$, 
% i.e., the exclusive base vectors for $\sn\{U^{3}\}$ and $\sn\{U^{4}\}$ are in $\sn\{U^{(1)}\}$ and $\sn\{U^{(2)}\}$, respectively, 
and  2) $n \leq Z + \min\{a, b\}$, then $\mathcal{L}_{\text{total,lb}}$ is achievable.
\end{theorem}

\input{figs_tex/explanation.tex}

For the clarity of the presentation, we only provide the proof when $2Z \leq n$. The proof idea for $2Z > n$ is quite similar and we put it in Section \ref{subsec:proof_thm_sf3} due to space limit.

\begin{proof}
% We first have $r_-^{(3,4)} \geq 2n -a - b$. This is because, 
% % 1) if $\min\{2Z, n\} = n$, we have $r_+^{(3,4)} = r_-^{(3,4)} = n$. Since $n \leq a+b$, we have $r_-^{(3,4)} = n \geq 2n -a -b$; 2) 
% % if $\min\{2Z, n\} = 2Z$, we have
% $n \leq Z + \min\{a, b\}$ and 
% $n + 2Z - r_-^{(3,4)} = n + r_+^{(3,4)} - 2Z \leq Z + \min\{a, b\}$. So $r_-^{(3,4)} \geq n - \min\{a, b\} + Z \geq 2 (n - \min\{a, b\}) \geq 2n -a - b$.

Suppose $2Z \leq n$.
We start with a matrix $W \in \reals^{r_-^{(3,4)} \times n}$. We use $w_{1}, w_{2}, \cdots, w_{r_-^{(3,4)}}$ to denote its row vectors, and initialize them by $v_{r_+^{(3,4)}-2Z+1}, \cdots, v_{2Z}$. That is:
\begin{align}
W =
\begin{bmatrix}
w^\top_{1}\\
w^\top_{2}\\
\vdots\\
w^\top_{r_-^{(3,4)}}
\end{bmatrix}
\leftarrow
\begin{bmatrix}
v_{r_+^{(3,4)}-2Z+1}^\top\\
v_{r_+^{(3,4)}-2Z+2}^\top\\
\vdots\\
v_{2Z}^\top
\end{bmatrix}.
\end{align}

We next do transformations on $W$, as shown in Fig. \ref{fig:explanation}. There are four major steps:

I) We put columns $a+1:n$ before columns $n-b+1:a$ for the convenience of further transformations.

II) We next perform Gauss-Jordan elimination over $W$, and get its reduced row echelon form, which has the following two properties:
i) The leading coefficient of a nonzero row is always strictly to the right of the leading coefficient of the row above it, and is always 1 (called a leading 1);
ii) Each column containing a leading 1 has zeros in all its other entries. 
Therefore, $W$ now must have the form as shown in Fig. \ref{fig:explanation} after Step II, where $a'$ and $b'$ are integers such that $a \leq a' \leq n$, $b \leq b' \leq n$ and . Here without loss of generality, we assume that the first $p$ columns for columns $a+1:n$ do not have leading 1, where $p \leq n -a' \leq n -a \leq Z$. And $a', b', p$ also satisfy $r_-^{(3,4)} + a'+b'+p-2n \geq 0$. 
% Note that columns $1:n-b$ may or may not have leading 1 but we don't differentiate. 

III) We put columns $a+1:n$ before columns $1:n-b$, and then perform Gauss-Jordan elimination for the first $n-b'$ rows. $W$ now has the form as shown in Fig. \ref{fig:explanation} after Step III.

IV) We rearrange the columns in their original order.  $W$ now has the form as shown in Fig. \ref{fig:explanation} after Step IV. And for convenience we divide the row vectors of $W$, $w_{1}, w_{2}, \cdots, w_{r_-^{(3,4)}}$, into 4 groups denoted by $G_1$, $G_2$, $G_3$ and $G_4$ respectively. We have $|G_1| = \min\{p, n-b'\}$, $|G_2| = \max\{n-b'-p,0\}$, $|G_3| = n-a'-p$ and $|G_4| = r_-^{(3,4)} + a'+b'+p-2n$. And note that $|G_1| + \max\{|G_2|, |G_3|\} \leq n - \min\{a', b'\} \leq Z$.

% V) We divide the row vectors of $W$, $w_{1}, w_{2}, \cdots, w_{r_-^{(3,4)}}$, into 4 groups, as shown in Fig. \ref{fig:explanation} after Step V. Here group 1 has $\min\{p, n -b'\}$ vectors which depend on both $x^{(1)}$ and $x^{(2)}$ in general; group 2 and group 3 both has $\max\{n-a'-p, n -b'-p\}$ vectors which depend only on $x^{(1)}$ and $x^{(2)}$, respectively; and group 4 has $r_-^{(3,4)} + a'+b'+p-2n - |n-a'-p - \max\{n-b'-p, 0\}|$ vectors which depend only on the intersection of $x^{(1)}$ and $x^{(2)}$.

Note that after the whole transformation, $\sn\{W^\top\} = \sn\{v_{r_+^{(3,4)}-2Z+1}, v_{r_+^{(3,4)}-2Z+2}, \cdots, v_{2Z}\}$ remains unchanged.

% 1) Group 1 has $w_{1}, \cdots, w_{\min\{p, n -b'\}}$, which constitute the first row of blocks; 
% 2) Group 2 has $w_{\min\{p, n -b'\}+1}, \cdots, w_{n-b'}$, which constitute the second row of blocks, and $w_{2n-a'-b'-p+1}, \cdots, w_{n+Z-a'-p}$, which are the first $Z-n+b'$ rows of the fourth row of blocks; 
% 3) Group 3 has $w_{n-b'+1}, \cdots, w_{2n-a'-b'-p}$, which constitute the third row of blocks, and $w_{n+Z-a'-p+1}, \cdots, w_{2Z-\min\{p,n-b'\}}$, which are the first $Z-n+b'+1$ to $2Z-2n+a'+b'+p-\min\{p,n-b'\}$ rows ($Z-n+a'+p-\min\{p,n-b'\}$ in total) of the fourth row of blocks; 
% 4) Group 4 has $w_{2Z-\min\{p,n-b'\}+1}, \cdots, w_{r^{(3,4)}_-}$, which are the last $r^{(3,4)}_- - 2Z+\min\{p,n-b'\}$ rows of the fourth row of blocks.
% In summary, group 1 has $\min\{p, n -b'\}$ vectors which depend on both $x^{(1)}$ and $x^{(2)}$; group 2 and group 3 both has $Z - \min\{p, n -b'\}$ vectors which depend only on $x^{(1)}$ and $x^{(2)}$, respectively; and group 4 has $Z-n+a'+p-\min\{p,n-b'\}$ vectors which depend only on the intersection of $x^{(1)}$ and $x^{(2)}$.


We are able to find a network coding scheme such that $\mathcal{L}_{\text{total,lb}}$ is achievable. The scheme is:

1) Let the first $|G_1|$ column vectors of $\Phi^{(6,3)} = \Phi^{(6,4)}$ be the vectors in $G_1$, and there are $Z-|G_1|$ column vectors of $\Phi^{(6,3)} = \Phi^{(6,4)}$ to be determined;

2) Let the first $r_+^{(3,4)}-2Z$ column vectors of $\Phi^{(1,3)}$ and $\Phi^{(2,4)}$ be $v_1, \cdots, v_{r_+^{(3,4)}-2Z}$ and $v_{2Z+1}, \cdots, v_{r_+^{(3,4)}}$ respectively, and there are $3Z - r_+^{(3,4)}$ column vectors of $\Phi^{(1,3)}$ and $\Phi^{(2,4)}$ to be determined;

3.1) If $\min\{|G_2|, |G_3|\} > 3Z - r_+^{(3,4)}$, then let the non-determined column vectors of $\Phi^{(1,3)}$ and $\Phi^{(2,4)}$ be the first $3Z - r_+^{(3,4)}$ vectors in $G_2$ and $G_3$ respectively. Next let $3Z - r_+^{(3,4)}$ non-determined column vectors of $\Phi^{(6,3)} = \Phi^{(6,4)}$ be the pair-wise sums of the first $3Z - r_+^{(3,4)}$ vectors in $G_2$ and $G_3$. And in the end let the remaining non-determined column vectors of $\Phi^{(6,3)} = \Phi^{(6,4)}$ be the remaining vectors in $G_2$, $G_3$ and $G_4$;

3.2) If $\min\{|G_2|, |G_3|\} \leq 3Z - r_+^{(3,4)}$, then let $\min\{|G_2|, |G_3|\}$ non-determined column vectors of $\Phi^{(1,3)}$ and $\Phi^{(2,4)}$ be the first $\min\{|G_2|, |G_3|\}$ vectors in $G_2$ and $G_3$ respectively. Next let $\min\{|G_2|, |G_3|\}$ non-determined column vectors of $\Phi^{(6,3)} = \Phi^{(6,4)}$ be the element-wise sum of the first $\min\{|G_2|, |G_3|\}$ vectors in $G_2$ and $G_3$, and another $\max\{|G_2|, |G_3|\}-\min\{|G_2|, |G_3|\}$ non-determined column vectors of $\Phi^{(6,3)} = \Phi^{(6,4)}$ be the remaining vectors in $G_2$ or $G_3$. In the end let the remaining non-determined column vectors of $\Phi^{(6,3)} = \Phi^{(6,4)}$ be the first $Z-|G_1| - \max\{|G_2|, |G_3|\}$ vectors in $G_4$, and the remaining non-determined column vectors of $\Phi^{(1,3)}$ and $\Phi^{(2,4)}$ both be the remaining vectors in $G_4$.

% 3) Let the last $Z-\min\{p, n -b'\}-\max\{n-a'-p, n -b'-p\}$ column vectors of $\Phi^{(6,3)} = \Phi^{(6,4)}$ be the first $Z-\min\{p, n -b'\}-\max\{n-a'-p, n -b'-p\}$ vectors in group 4; 
% 4) Let the column vectors of $\Phi^{(1,3)}$ be the remaining vectors in group 4, all the vectors in group 2, and $v_1, \cdots, v_{r_+^{(3,4)}-2Z}$, and the column vectors of $\Phi^{(2,4)}$ be the remaining vectors in group 4, all the vectors in group 3, and $v_{2Z+1}, \cdots, v_{r_+^{(3,4)}}$. 
It can be verified that $\sn\{W^\top\} \subset \sn\{[\Phi^{(1,3)}, \Phi^{(6,3)}]\}$ and $\sn\{W^\top\} \subset \sn\{[\Phi^{(2,4)}, \Phi^{(6,4)}]\}$. Furthermore, $\sn\{U^{(3)}\} = \sn\{[\Phi^{(1,3)}, \Phi^{(6,3)}]\}$ and $\sn\{U^{(4)}\} = \sn\{[\Phi^{(2,4)}, \Phi^{(6,4)}]\}$. Therefore, $\mathcal{L}_{\text{total,lb}}$ is achievable.
\end{proof}


% is: 1) Let the column vectors of $\Phi^{(6,3)} = \Phi^{(6,4)}$ be composed of the the vectors in group 1 and the element-wise sum of the vectors in group 2 and group 3; 2) Let the column vectors of $\Phi^{(1,3)}$ be the vectors in group 2, group 4 and $v_1, \cdots, v_{r_+^{(3,4)}-\min\{2Z, n\}}$; 3) Let the column vectors of $\Phi^{(2,4)}$ be the vectors in group 3, group 4 and $v_{\min\{2Z, n\}+1}, \cdots, v_{r_+^{(3,4)}}$. Node 3 can decode all the row vectors of $W$, and hence can also decode $v_{r_+^{(3,4)}-\min\{2Z, n\}+1}, \cdots, v_{\min\{2Z, n\}}$. Thus node 3 can decode $v_1, \cdots, v_{\min\{2Z, n\}}$. Similarly, node 4 can decode $v_{r_+^{(3,4)}-\min\{2Z, n\}+1}, \cdots, v_n$.

\begin{corollary}\label{cor:sf3}
If $S^{(3)} = S^{(4)}$, that is, the tasks are the same, and $n \leq Z + \min\{a, b\}$, then $\mathcal{L}_{\text{total,lb}}$ is achievable.
\end{corollary}


==> sections/old/butterfly.tex <==
\input{figs_tex/architecture2.tex}

Two data sources possess $x_1, x_2 \in \reals^{m}$, respectively. Suppose the original and full data is $x \in \reals^n$, where $m \leq n \leq 2m$. When $n = m$, $x_1 = x_2$; when $n = 2m$, $x_1$ and $x_2$ are independent; and otherwise $x_1$ and $x_2$ are partially correlated.

Each destination has a machine learning task. When these tasks are linear inferences there are task matrices $K_3$ and $K_4$. We say they are the same if $K_3=K_4$; they are independent if for any pairs of eigen-vectors of $K_3$ and $K_4$, denoted by $e_3$ and $e_4$, if they both correspond to non-zero eigen values, $e_3 \perp e_4$; otherwise they are partially correlated.

\begin{table*}[ht]
\caption{.}
\label{tab:}
\vskip 0.15in
\begin{center}
\resizebox{2\columnwidth}{!}{
\begin{tabular}{lcccr}
\toprule
Tasks $\setminus$ Sources & Same ($n=m$) & Independent ($n=2*m$) & Correlated ($m < n < 2*m$)\\
\midrule
Same & top-$2Z$ of $K_3=K_4$ & top-$2Z$ in each space &  top-$\min\{2Z, n\}$ achievable for $n \leq m+ Z$ \\
Independent &  top-$3Z$ (each at most $2Z$) of $K_3$ and $K_4$ & top-$3Z$ of $K_3$ and $K_4$ over subspaces&  \\
Correlated &  top-$\min\{2Z, n\}$ achievable of $K_3$ and $K_4$ achievable if $n \leq 3Z$ &  &  ?\\
\bottomrule
\end{tabular}
}
\end{center}
\vskip -0.1in
\end{table*}

==> sections/old/evaluation.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.5]{figs/result_1.pdf}
\caption{Result 1.}
\label{fig:result_1}
\end{figure}

Fig. \ref{fig:result_1} shows our evaluation result. In our simulation, we use MNIST dataset. Each data point is a $28 \times 28$ image, i.e., $n = 784$. We consider a network with $k = 16$, $m = 49$ and $r = 1$. We consider $Z = 2, 4, 6, 8$.

The considered algorithms are:
1) Codesign -- our algorithm;
2) Leaf first -- Train the sensor encoders first (with task agnostic loss), then train the edge encoder (with overall task loss);
3) Root first -- Train the edge encoder first (with overall task loss and assume sensor-edge channels are not bottlenecked), then train the sensor encoders (with task agnostic loss);
4) Task-agnostic -- codesign with task-agnostic loss.



==> sections/old/problem_formulation.tex <==
\input{figs_tex/architecture.tex}

We now formulate the problem of task-aware data compression over bottlenecked networks as shown in Fig. \ref{fig:architecture}. 

In the problem, there are $k$ sensors indexed by $1, 2, \cdots, k$, respectively. Let $x \in \reals^n$ be the full observation of all the sensors, and $x_i \in \reals^m$ be the partial observation of sensor $i$, $\forall i$. Here we assume the observations of different sensors are independent, i.e., $n = km$ and $x = [x_1^\top, x_1^\top, \cdots, x_k^\top]^\top$. We let $x_i = P_i x$, where $P_i \in \reals^{m \times n}$ is an immutable binary matrix, with $P_i P_i^\top = I$ and $P_i P_j^\top = \bm{0}$.

All the sensors considered are connected to the same edge server. Due to the rate limit of the channels between the sensor and the edge server, sensor $i$ has to encode $x_i$ as $\phi_i \in \reals^r$, through encoder function $g_e^i: \reals^m \mapsto \reals^r$ (which is lossy in general) as follows:
\begin{align}
\phi_i = g_e^i(x_i; \theta_e^i), \quad \forall i \in \{1, 2, \cdots, k\}
\end{align}
where $\theta_e^i$ is the encoder parameter. The edge server aggregates the encoded partial observations to $\phi = [\phi_1^\top, \phi_2^\top, \cdots, \phi_k^\top]^\top \in \reals^{kr}$.

Next, the edge server uploads the aggregated observation $\phi$ to the cloud. Due to the rate limit of the channels between the edge server and the cloud, the edge server has to encode $\phi$ as $\phi_0$, through encoder function $g_e^0: \reals^{kr} \mapsto \reals^Z$ (which is lossy in general) as follows:
\begin{align}
\phi_0 = g_e^0(\phi; \theta_e^0)
\end{align}
where $\theta_e^0$ is the encoder parameter.

The cloud receives $\phi_0$, and gives an estimation $\hat{x}$ of the full observation through decoder function $g_d: \reals^Z \mapsto \reals^n$ as follows:
\begin{align}
\hat{x} = g_d(\phi_0; \theta_d)
\end{align}
where $\theta_d$ is the decoder parameter. $\hat{x}$ will be used as the input for an inference task $f: \reals^n \mapsto \reals$ as follows:
\begin{align}
\hat{y} = f(\hat{x})
\end{align}
where $\hat{y}$ is the inference output. The task loss is defined as:
\begin{align}
\mathcal{L}_\text{task} = \E_x [l(y, \hat{y})]
\end{align}
where $y = f(x)$ is the inference output when $x$ is the input, and $l$ is a common loss function (e.g., squared-error distortion or cross entropy function) that measures the discrepancy between $y$ and $\hat{y}$. Our primary objective is to minimize $\mathcal{L}_\text{task}$ as much as possible. Moreover, our secondary objective is to recover the original observation as much as possible, and the associated reconstruction loss is defined as:
\begin{align}
\mathcal{L}_\text{recon} = \E_x [\|x - \hat{x}\|_2^2]
\end{align}

Therefore, we can write our overall objective as a weighted sum of $\mathcal{L}_\text{task}$ and $\mathcal{L}_\text{recon}$ as follows:
\begin{align}
\mathcal{L}_\text{total} = \mathcal{L}_\text{task} + \lambda \mathcal{L}_\text{recon}
\end{align}
where $\lambda$ is a weight coefficient. And the problem can be written as an optimization problem:
\begin{align}
\min_{\theta_e^i, \theta_d} \quad \mathcal{L}_\text{total}
\end{align}


==> sections/old/problem_formulation_2.tex <==
\input{figs_tex/architecture.tex}
\input{figs_tex/obs_tasks.tex}
We now formulate task-aware data compression problem over butterfly network, as shown in Fig. \ref{fig:architecture}. The butterfly network has 6 nodes indexed by $1, 2, \cdots, 6$, respectively. Here node 1 and 2 are data sources, node 3 and 4 are data destinations, and node 5 and 6 are intermediate nodes. 

\textbf{Data sources}. We have an original data vector $x = [x_1, x_2, \cdots, x_n]\in \reals^n$. Node 1 and 2 have immutable observations of $x$, denoted by $x^{(1)} = \in \reals^a$ and $x^{(2)} = \in \reals^b$, respectively. Here observations $x^{(1)}$ and $x^{(2)}$ are composed of $a$ and $b$ different dimensions of $x$, respectively; and each dimension of $x$ exists in \textit{at least} one of the two observations. Therefore, we have $\max\{a, b\} \leq n \leq a+b$. Without loss of generality, we let $x^{(1)} = [x_1, x_2, \cdots, x_{n-b}, x_{2n-a-b+1}, \cdots, x_n]$ and $x^{(2)} = [x_{n-b+1}, x_{n-b+2}, \cdots, x_n]$, that is, $x_{1:n-b}$ and $x_{n-b+1:2n-a-b}$ are node 1 and node 2's exclusive observations, and $x_{2n-a-b+1:n}$ are their mutual observations.

\textbf{Data transmission}. In the butterfly network there are 7 links, and each one transmits in the direction specified by the corresponding arrow. We use $(i, j)$ to denote a link with source node $i$ and destination node $j$. All the links have the same capacities, and in our problem we assume each can only transmit a variable in $\reals^Z$. Since we consider a bottlenecked butterfly network, we assume that $Z \leq \min\{a, b\}$. Here for each link $(i, j) \in E = \{(1,3), (1,5), (2,4), (2,5), (5,6)\}$
, since the overall number of input dimensions for node $i$ is larger than $Z$, we use an encoder function $g_e^{i,j}$ as follows:
\begin{align}
\phi^{(i,j)} = g_e^{i,j}(\cdot; \theta_e^{i,j}), \quad \forall (i, j) \in E
\end{align}
where the input of $g_e^{i,j}$ is the input or the aggregated input (i.e., concatenated vector) for node $i$, $\phi^{(i,j)} \in \reals^{Z}$ is the data that transmits over $(i, j)$, and $\theta_e^{i,j}$ is the parameter of $g_e^{i,j}$. For link $(6,3)$ and $(6,4)$, they simply transmit the data received by node 6, i.e., $\phi^{(6,3)} = \phi^{(6,4)} = \phi^{(5,6)}$.

\textbf{Data reconstruction}. Node 3 and 4 aim to reconstruct the original data $x$, through the aggregated inputs they received from their respective input links. The corresponding decoder function $g_d^i: \reals^{2Z} \mapsto \reals^{n}, \forall i \in \{3, 4\}$ is as follows:
\begin{align}
\hat{x}^{(i)} = g_d^i(\cdot; \theta_d^i), \quad \forall i \in \{3, 4\}
\end{align}
where the input of $g_d^i$ is the aggregated input for node $i$, $\hat{x}^{(i)}$ is the reconstructed data for node $i$, and $\theta_d^i$ is the parameter of $g_d^i$.


\textbf{Task objective}. Node $i$ ($\forall i \in \{3, 4\}$) use the reconstructed data $\hat{x}^{(i)}$ as the input for an inference task $f_i: \reals^n \mapsto \reals^{m_i}$ as follows:
\begin{align}
\hat{y}^{(i)} = f^i(\hat{x}^{(i)}), \quad \forall i \in \{3, 4\}
\end{align}
where $\hat{y}^{(i)} \in \reals^{m_i}$ is the inference output. The task loss is defined as:
\begin{align}
\mathcal{L}_{\text{task},i} = \E_x [l(y^{(i)}, \hat{y}^{(i)})], \quad \forall i \in \{3, 4\}
\end{align}
where $y^{(i)} = f_i(x)$ is the inference output when $x$ is the input, and $l$ is a common loss function (e.g., squared-error distortion or cross entropy function) that measures the discrepancy between $y^{(i)}$ and $\hat{y}^{(i)}$. Our primary objective is to minimize $\mathcal{L}_{\text{task},i}$ as much as possible. Moreover, our secondary objective is to recover the original data as much as possible, and the associated reconstruction loss is defined as:
\begin{align}
\mathcal{L}_{\text{recon},i} = \E_x [\|x - \hat{x}^{(i)}\|_2^2], \quad \forall i \in \{3, 4\}
\end{align}

Therefore, we can write our overall objective as a weighted sum of $\mathcal{L}_{\text{task},i}$ and $\mathcal{L}_{\text{recon},i}$ as follows:
\begin{align}
\mathcal{L}_\text{total} = \sum_{i=3,4}\mathcal{L}_{\text{task},i} + \lambda \sum_{i=3,4} \mathcal{L}_{\text{recon},i}
\end{align}
where $\lambda$ is a weight coefficient. 

\textbf{Task-aware data compression problem}. The problem can be written as an optimization problem:
\begin{align}
\min_{\theta_e^{i,j}, \theta_d^{i}} \quad \mathcal{L}_\text{total}
\end{align}

